Search for excited electrons singly produced in proton-proton collisions at $\sqrt{s} = 13$ TeV with the ATLAS experiment at the LHC

A search for excited electrons produced in $pp$ collisions at $\sqrt{s} = 13$ TeV via a contact interaction $q\bar{q} \to ee^*$ is presented. The search uses 36.1 fb$^{-1}$ of data collected in 2015 and 2016 by the ATLAS experiment at the Large Hadron Collider. Decays of the excited electron via a contact interaction into an electron and a pair of quarks ($eq\bar{q}$) are targeted in final states with two electrons and two hadronic jets, and decays via a gauge interaction into a neutrino and a $W$ boson ($\nu W$) are probed in final states with an electron, missing transverse momentum, and a large-radius jet consistent with a hadronically decaying $W$ boson. No significant excess is observed over the expected backgrounds. Upper limits are calculated for the $pp \to ee^* \to eeq\bar{q}$ and $pp \to ee^* \to e\nu W$ production cross sections as a function of the excited electron mass $m_{e^*}$ at 95% confidence level. The limits are translated into lower bounds on the compositeness scale parameter $\Lambda$ of the model as a function of $m_{e^*}$. For $m_{e^*} < 0.5$ TeV, the lower bound for $\Lambda$ is 11 TeV. In the special case of $m_{e^*} = \Lambda$, the values of $m_{e^*} < 4.8$ TeV are excluded. The presented limits on $\Lambda$ are more stringent than those obtained in previous searches.

==> EXOT-2017-22-PAPER-hepdata.tex <==
\section{HepData material}
%-------------------------------------------------------------------------------

This file is available for detailed tables etc.\ that are going to be
submitted to HepData or other similar destinations.

==> yieldsTCR_formatted.tex <==
\begin{sidewaystable}
	\caption{Event yields in the \ttbar control regions of the \eejj channel. Data are shown together with the background contributions after constraint in control regions.}
	\label{yields:table:TCR:CI}
	\begin{center}
	\setlength{\tabcolsep}{0.2pc}
		{
		\small
			\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c}
				\hline
				\textbf{Yields}                  & CR1           & CR2           & CR3           & CR4           & CR5             & CR6             & CR7             & CR8             & CR9             & CR10  \\
				\hline
Observed & $468$ & $71$ & $66$ & $45$ & $30$ & $29$ & $19$ & $17$ & $12$ & $16$ \\
\hline
Background & $470\pm20$ & $71\pm8$ & $66\pm8$ & $45\pm7$ & $30\pm6$ & $29\pm5$ & $19\pm4$ & $17\pm4$ & $12\pm4$ & $16\pm4$ \\
\hline
$t\bar{t}$ & $390\pm20$ & $49\pm9$ & $37\pm9$ & $22\pm7$ & $17\pm6$ & $17\pm6$ & $8\pm5$ & $7\pm4$ & $6\pm4$ & $10\pm4$ \\
Single-top (Wt) & $51\pm2$ & $14.2\pm1.0$ & $18.7\pm1.2$ & $15.1\pm1.1$ & $7.5\pm0.7$ & $7.5\pm0.7$ & $6.4\pm0.7$ & $5.6\pm0.8$ & $3.5\pm0.4$ & $2.2\pm0.2$ \\
Diboson & $29\pm8$ & $8\pm2$ & $10\pm3$ & $8\pm2$ & $5.1\pm1.4$ & $4.8\pm1.3$ & $4.6\pm1.3$ & $4.0\pm1.1$ & $2.8\pm0.8$ & $3.6\pm1.0$ \\
$Z/\gamma*\rightarrow \tau\tau$ & $0.8\pm1.0$ & $0.07\pm0.02$ & $0.04\pm0.02$ & $0.04\pm0.02$ & $0.020\pm0.010$ & $0.030\pm0.010$ & $0.05\pm0.02$ & $0.06\pm0.02$ & $0.020\pm0.010$ & $0.040\pm0.010$ \\
				\hline
			\end{tabular}
		}
	\end{center}
\end{sidewaystable}

==> yieldsTCR_formatted_GI.tex <==
\begin{sidewaystable}
	\caption{Event yields in the \ttbar control regions of the \enuJ channel. Data are shown together with the background contributions after constraint in control regions.}
	\label{yields:table:TCR:GI}
	\begin{center}
	\setlength{\tabcolsep}{0.2pc}
		{
		\small
			\begin{tabular}{l|c|c|c|c|c|c|c|c|c}
				\hline
				\textbf{Yields} & CR1 & CR2 & CR3 & CR4 & CR5 & CR6 & CR7 & CR8 & CR9  \\
				\hline
Observed & $48$ & $73$ & $94$ & $54$ & $62$ & $29$ & $9$ & $10$ & $4$ \\
\hline
Background & $48\pm7$ & $73\pm9$ & $94\pm10$ & $54\pm8$ & $62\pm8$ & $29\pm6$ & $9\pm3$ & $10\pm3$ & $4\pm2$ \\
\hline
$W\rightarrow e\nu$ & $0.3\pm0.2$ & $4\pm3$ & $5\pm3$ & $5\pm4$ & $5\pm4$ & $5\pm4$ & $4\pm3$ & $0.11\pm0.12$ & $0.04\pm0.03$ \\
$Z/\gamma^*\rightarrow ee$ & $0.3\pm0.2$ & $0.30\pm0.11$ & $0.4\pm0.2$ & $0.15\pm0.14$ & $0.2\pm0.2$ & $0.10\pm0.05$ & $0.04\pm0.04$ & $0.02\pm0.02$ & $0.010\pm0.010$ \\
$t\bar{t}$ & $47\pm7$ & $64\pm9$ & $79\pm11$ & $41\pm9$ & $46\pm9$ & $15\pm7$ & $1\pm2$ & $7\pm4$ & $4\pm2$ \\
Single-top & $0.4\pm0.5$ & $2.5\pm1.1$ & $4.8\pm1.3$ & $6\pm2$ & $6\pm2$ & $6\pm2$ & $2.6\pm1.4$ & $1.1\pm0.5$ & $0.4\pm0.3$ \\
Fake electron & \--- & $2.2\pm0.8$ & $5\pm2$ & $2.0\pm0.8$ & $5\pm2$ & $2.5\pm0.9$ & $1.8\pm0.7$ & $1.6\pm0.6$ & \--- \\
Diboson & \--- & \--- & \--- & $0.13\pm0.06$ & $0.13\pm0.10$ & $0.13\pm0.10$ & \--- & \--- & \--- \\
$Z/\gamma^*\rightarrow \tau\tau$ & \--- & $0.02\pm0.02$ & $0.06\pm0.03$ & $0.04\pm0.02$ & $0.04\pm0.02$ & $0.020\pm0.010$ & \--- & \--- & \--- \\
				\hline
			\end{tabular}
		}
	\end{center}
\end{sidewaystable}

==> yieldsTVR_formatted_GI_bkgonly.tex <==
\begin{sidewaystable}
	\caption{Event yields in the $b$-jet validation regions of the \enuJ channel. Data are shown together with the background contributions after constraint in control regions.}
	\label{yields:table:TVR_bkgonly:GI}
	\begin{center}
	\setlength{\tabcolsep}{0.2pc}
		{
		\small
			\begin{tabular}{l|c|c|c|c|c|c|c|c|c}
				\hline
				\textbf{Yields} & VR1 & VR2 & VR3 & VR4 & VR5 & VR6 & VR7 & VR8 & VR9  \\
				\hline
Observed & $28$ & $53$ & $64$ & $34$ & $35$ & $27$ & $10$ & $4$ & $1$ \\
\hline
Background & $28\pm6$ & $42\pm9$ & $54\pm11$ & $33\pm9$ & $51\pm13$ & $25\pm9$ & $6\pm2$ & $14\pm8$ & $8\pm6$ \\
\hline
$W\rightarrow e\nu$ & $0.9\pm0.3$ & $1.4\pm0.6$ & $2.8\pm1.0$ & $2.6\pm0.8$ & $4\pm2$ & $3.3\pm0.9$ & $0.6\pm0.9$ & $0.6\pm0.3$ & $0.13\pm0.09$ \\
$Z/\gamma^*\rightarrow ee$ & $0.5\pm0.6$ & $0.9\pm0.6$ & $1.3\pm0.6$ & $1.0\pm0.5$ & $1.1\pm0.5$ & $0.4\pm0.2$ & $0.15\pm0.08$ & $0.09\pm0.05$ & $0.02\pm0.02$ \\
$t\bar{t}$ & $19\pm5$ & $32\pm8$ & $40\pm9$ & $22\pm8$ & $36\pm12$ & $12\pm7$ & $0.5\pm1.5$ & $11\pm8$ & $6\pm6$ \\
Single-top & $2.8\pm0.9$ & $7\pm3$ & $8\pm3$ & $7\pm3$ & $9\pm4$ & $5\pm5$ & $3.5\pm1.2$ & $2.2\pm0.6$ & $1.8\pm1.3$ \\
Fake electron& $5\pm2$ & $0.42\pm0.10$ & $1.4\pm0.5$ & \--- & \--- & $3.5\pm1.4$ & $1.6\pm0.7$ & $0.08\pm0.02$ & $0.18\pm0.06$ \\
Diboson & $0.1\pm0.4$ & $0.7\pm0.7$ & $0.7\pm1.1$ & $0.1\pm0.3$ & $1.4\pm1.5$ & $0\pm2$ & \--- & \--- & \--- \\
$W\rightarrow \tau\nu$ & \--- & \--- & $0.01\pm0.02$ & $0.01\pm0.06$ & $0.2\pm0.2$ & $0.10\pm0.02$ & \--- & \--- & \--- \\
$Z/\gamma^*\rightarrow \tau\tau$ & \--- & $0.0\pm0.2$ & $0.0\pm0.2$ & $0.010\pm0.010$ & $0.03\pm0.02$ & $0.010\pm0.010$ & $0.000\pm0.010$ & \--- & \--- \\
\hline
			\end{tabular}
		}
	\end{center}
\end{sidewaystable}

==> yieldsWCR_formatted_GI.tex <==
\begin{sidewaystable}
	\caption{Event yields in the $W$ control regions of the \enuJ channel. Data are shown together with the background contributions after constraint in control regions. The second and the third \Wboson CRs are identical and combined into the one column, as they differ according to the \absdphienu requirement, which is not applied for the \Wboson control regions.}
	\label{yields:table:WCR:GI}
	\begin{center}
	\setlength{\tabcolsep}{0.2pc}
		{
		\small
			\begin{tabular}{l|c|c|c|c|c|c|c|c}
				\hline
				\textbf{Yields} & CR2/CR3 & CR4 & CR5 & CR6 & CR7 & CR8 & CR9  \\
				\hline
Observed & $9198$ & $9168$ & $9090$ & $7312$ & $4760$ & $2903$ & $1834$ \\
\hline
Background & $9200\pm100$ & $9170\pm100$ & $9090\pm100$ & $7310\pm90$ & $4800\pm300$ & $2900\pm60$ & $1830\pm50$ \\
\hline
$W\rightarrow e\nu$ & $5900\pm400$ & $5700\pm600$ & $5300\pm600$ & $4900\pm400$ & $3500\pm500$ & $1600\pm400$ & $1000\pm300$ \\
$Z/\gamma^*\rightarrow ee$ & $24\pm13$ & $19\pm11$ & $14\pm8$ & $10\pm5$ & $6\pm3$ & $4\pm2$ & $2.1\pm0.9$ \\
$t\bar{t}$ & $1200\pm300$ & $1300\pm500$ & $1700\pm600$ & $700\pm400$ & $100\pm200$ & $500\pm400$ & $300\pm200$ \\
Single-top & $210\pm20$ & $200\pm20$ & $200\pm20$ & $149\pm11$ & $97\pm6$ & $61\pm5$ & $40\pm4$ \\
Fake electron & $460\pm120$ & $450\pm120$ & $430\pm110$ & $370\pm90$ & $220\pm50$ & $140\pm40$ & $80\pm20$ \\
Diboson & $560\pm110$ & $550\pm110$ & $550\pm110$ & $450\pm100$ & $310\pm70$ & $200\pm40$ & $120\pm30$ \\
$W\rightarrow \tau\nu$ & $800\pm200$ & $800\pm200$ & $800\pm200$ & $700\pm200$ & $460\pm110$ & $310\pm80$ & $210\pm60$ \\
$Z/\gamma^*\rightarrow \tau\tau$ & $160\pm50$ & $160\pm50$ & $160\pm50$ & $120\pm30$ & $80\pm20$ & $50\pm20$ & $28\pm8$ \\
\hline
			\end{tabular}
		}
	\end{center}
\end{sidewaystable}

==> yieldsWVR_formatted_GI_bkgonly.tex <==
\begin{sidewaystable}
	\caption{Event yields in the \mJ validation regions of the \enuJ channel. Data are shown together with the background contributions after constraint in control regions.}
	\label{yields:table:WVR_bkgonly:GI}
	\begin{center}
	\setlength{\tabcolsep}{0.2pc}
		{
		\small
			\begin{tabular}{l|c|c|c|c|c|c|c|c|c}
				\hline
				\textbf{Yields} & VR1 & VR2 & VR3 & VR4 & VR5 & VR6 & VR7 & VR8 & VR9  \\
				\hline
Observed & $31$ & $58$ & $72$ & $33$ & $46$ & $35$ & $14$ & $11$ & $6$ \\
\hline
Background & $30\pm6$ & $50\pm9$ & $64\pm11$ & $36\pm14$ & $47\pm12$ & $23\pm8$ & $6\pm3$ & $10\pm5$ & $4\pm2$ \\
\hline
$W\rightarrow e\nu$ & $2.0\pm1.2$ & $5.8\pm1.5$ & $7\pm2$ & $6\pm2$ & $11\pm6$ & $5\pm4$ & $4\pm2$ & $2.7\pm1.3$ & $0.9\pm0.9$ \\
$Z/\gamma^*\rightarrow ee$ & $1.1\pm0.7$ & $1.8\pm0.9$ & $2.2\pm1.1$ & $1.0\pm0.5$ & $1.2\pm0.7$ & $0.8\pm0.4$ & $0.20\pm0.11$ & $0.11\pm0.07$ & $0.05\pm0.03$ \\
$t\bar{t}$ & $22\pm6$ & $35\pm9$ & $46\pm11$ & $22\pm13$ & $30\pm10$ & $11\pm6$ & $1\pm2$ & $6\pm5$ & $3\pm2$ \\
Single-top & $1.4\pm0.8$ & $2.4\pm0.8$ & $3.3\pm1.3$ & $3\pm2$ & $3.3\pm1.3$ & $2.7\pm1.1$ & $0.4\pm0.5$ & \--- & \--- \\
Fake electron & $2.0\pm0.3$ & $2.1\pm0.5$ & $2.6\pm0.5$ & $2.8\pm1.3$ & $0.7\pm0.6$ & $4\pm2$ & \--- & \--- & \--- \\
Diboson & $1.0\pm0.7$ & $2\pm2$ & $3\pm2$ & $1.7\pm1.3$ & $0.6\pm0.7$ & $0.0\pm0.8$ & \--- & $0.3\pm0.2$ & $0.2\pm0.2$ \\
$W\rightarrow \tau\nu$ & \--- & \--- & $0.22\pm0.13$ & $0.2\pm0.2$ & $0.22\pm0.13$ & $0.26\pm0.12$ & $0.26\pm0.12$ & $0.27\pm0.13$ & $0.04\pm0.08$ \\
$Z/\gamma^*\rightarrow \tau\tau$ & \--- & \--- & $0.02\pm0.02$ & $0.04\pm0.03$ & $0.02\pm0.07$ & $0.05\pm0.05$ & $0.03\pm0.06$ & $0.010\pm0.010$ & $0.010\pm0.010$ \\
\hline
			\end{tabular}
		}
	\end{center}
\end{sidewaystable}

==> yieldsZCR_formatted.tex <==
\begin{sidewaystable}
	\caption{Event yields in the \zgamma control regions of the \eejj channel. Data are shown together with the background contributions after constraint in control regions.}
	\label{yields:table:ZCR:CI}
	\begin{center}
	\setlength{\tabcolsep}{0.2pc}
		{
		\small
			\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c}
				\hline
				\textbf{Yields}                  & CR1           & CR2           & CR3           & CR4           & CR5             & CR6             & CR7             & CR8             & CR9             & CR10  \\
				\hline
Observed & $38530$ & $3123$ & $1907$ & $1355$ & $699$ & $502$ & $275$ & $230$ & $132$ & $74$ \\
\hline
Background & $38500\pm200$ & $3120\pm60$ & $1910\pm40$ & $1360\pm40$ & $700\pm30$ & $500\pm20$ & $280\pm20$ & $230\pm20$ & $132\pm12$ & $74\pm9$ \\
\hline
$Z/\gamma^*\rightarrow ee$ & $35400\pm400$ & $2850\pm70$ & $1750\pm50$ & $1240\pm40$ & $640\pm30$ & $460\pm20$ & $250\pm20$ & $210\pm20$ & $118\pm12$ & $67\pm9$ \\
$t\bar{t}$ & $1090\pm120$ & $52\pm14$ & $20\pm6$ & $13\pm5$ & $9\pm3$ & $6\pm2$ & $1.1\pm0.9$ & $1.4\pm1.1$ & $1.6\pm1.1$ & $0.16\pm0.08$ \\
Single-top (Wt) & $86\pm3$ & $4.9\pm0.2$ & $1.5\pm0.2$ & $0.63\pm0.12$ & $0.12\pm0.12$ & \--- & \--- & \--- & \--- & \--- \\
Fake electron & $600\pm200$ & $60\pm20$ & $35\pm11$ & $24\pm7$ & $13\pm4$ & $9\pm3$ & $3.7\pm0.9$ & $3.4\pm0.9$ & $2.4\pm0.6$ & $1.6\pm0.4$ \\
Diboson & $1300\pm300$ & $160\pm40$ & $100\pm20$ & $80\pm20$ & $42\pm10$ & $30\pm8$ & $17\pm4$ & $14\pm3$ & $9\pm2$ & $5.4\pm1.5$ \\
$Z/\gamma^*\rightarrow \tau\tau$ & $13\pm4$ & $1.2\pm0.4$ & $0.8\pm0.3$ & $0.5\pm0.2$ & $0.21\pm0.07$ & $0.14\pm0.05$ & $0.13\pm0.05$ & $0.13\pm0.06$ & $0.07\pm0.03$ & $0.05\pm0.02$ \\
				\hline
			\end{tabular}
		}
	\end{center}
\end{sidewaystable}

==> yieldsmllVR_formatted.tex <==
\begin{sidewaystable}
	\caption{Event yields in the \mll validation regions of the \eejj channel. Data are shown together with the background contributions after constraint in control regions. Low and high \etmiss regions are separated by $\etmiss = 200$~GeV (VR2-VR4), $250$~GeV (VR5-VR6), $300$~GeV (VR7-VR8) and $350$~GeV (VR9-VR10).
	}
	\label{yields:table:mllVR:CI}
	\begin{center}
	\setlength{\tabcolsep}{0.2pc}
		{
		\small
			\begin{tabular}{c|l|c|c|c|c|c|c|c|c|c}
\hline
& \textbf{Yields}                  & VR1           & VR2           & VR3           & VR4           & VR5             & VR6             & VR7             & VR8             & VR9 \\
\hline
\multirow{8}{*}{\rot{Integral}} & Observed & $9694$ & $538$ & $282$ & $208$ & $114$ & $80$ & $33$ & $28$ & $17$ \\
\cline{2-11}
& Background & $9770\pm90$ & $590\pm40$ & $320\pm20$ & $230\pm20$ & $112\pm8$ & $74\pm6$ & $29\pm3$ & $25\pm3$ & $16\pm2$ \\
\cline{2-11}
& $Z/\gamma^*\rightarrow ee$ & $2600\pm20$ & $233\pm10$ & $138\pm6$ & $99\pm5$ & $53\pm4$ & $37\pm3$ & $18\pm2$ & $15\pm2$ & $8.9\pm1.2$ \\
& $t\bar{t}$ & $5860\pm80$ & $210\pm40$ & $100\pm20$ & $67\pm12$ & $25\pm6$ & $15\pm5$ & $3\pm3$ & $3\pm2$ & $2\pm2$ \\
& Single-top (Wt) & $520\pm3$ & $49\pm2$ & $24\pm2$ & $18.9\pm1.2$ & $10.0\pm0.6$ & $5.8\pm0.4$ & $1.4\pm0.4$ & $1.3\pm0.4$ & $0.6\pm0.3$ \\
& Fake electron & $432\pm2$ & $52\pm11$ & $28\pm6$ & $21\pm4$ & $12\pm2$ & $7.9\pm1.1$ & $2.9\pm0.4$ & $2.6\pm0.5$ & $2.2\pm0.3$ \\
& Diboson & $349\pm2$ & $48\pm13$ & $29\pm8$ & $22\pm6$ & $12\pm3$ & $8\pm2$ & $3.7\pm1.1$ & $3.3\pm0.9$ & $2.3\pm0.7$ \\
& $Z/\gamma^*\rightarrow \tau\tau$ & $5.81\pm0.06$ & $0.5\pm0.2$ & $0.25\pm0.09$ & $0.21\pm0.09$ & $0.15\pm0.05$ & $0.08\pm0.03$ & $0.05\pm0.02$ & $0.05\pm0.02$ & $0.030\pm0.010$ \\
\hline
\multirow{8}{*}{\rot{Low \etmiss}} & Observed & \--- & $473$ & $248$ & $180$ & $106$ & $76$ & $32$ & $28$ & $17$ \\
\cline{2-11}
& Background & \--- & $510\pm40$ & $270\pm20$ & $187\pm12$ & $98\pm7$ & $66\pm5$ & $27\pm3$ & $23\pm3$ & $15\pm2$ \\
\cline{2-11}
& $Z/\gamma^*\rightarrow ee$ & \--- & $223\pm9$ & $130\pm6$ & $92\pm5$ & $51\pm4$ & $36\pm3$ & $18\pm2$ & $15\pm2$ & $8.9\pm1.2$ \\
& $t\bar{t}$ & \--- & $170\pm30$ & $82\pm13$ & $50\pm9$ & $19\pm5$ & $11\pm4$ & $2\pm2$ & $2\pm2$ & $1.7\pm1.4$ \\
& Single-top (Wt) & \--- & $33\pm2$ & $14.3\pm1.4$ & $10.9\pm0.9$ & $6.9\pm0.5$ & $3.7\pm0.3$ & $0.9\pm0.4$ & $0.8\pm0.4$ & $0.2\pm0.2$ \\
& Fake electron & \--- & $45\pm9$ & $24\pm5$ & $18\pm3$ & $11\pm2$ & $7.8\pm1.1$ & $3.0\pm0.4$ & $2.6\pm0.5$ & $2.2\pm0.3$ \\
& Diboson & \--- & $39\pm11$ & $24\pm7$ & $17\pm5$ & $10\pm3$ & $7\pm2$ & $3.3\pm1.0$ & $2.9\pm0.8$ & $2.2\pm0.6$ \\
& $Z/\gamma^*\rightarrow \tau\tau$ & \--- & $0.38\pm0.13$ & $0.22\pm0.08$ & $0.18\pm0.08$ & $0.13\pm0.05$ & $0.08\pm0.03$ & $0.05\pm0.02$ & $0.04\pm0.02$ & $0.030\pm0.010$ \\
\hline
\multirow{8}{*}{\rot{High \etmiss}} & Observed & \--- & $65$ & $34$ & $28$ & $8$ & $4$ & $1$ & $0$ & $0$ \\
\cline{2-11}
& Background & \--- & $79\pm8$ & $49\pm5$ & $41\pm4$ & $13\pm2$ & $9\pm2$ & $1.8\pm0.7$ & $1.7\pm0.7$ & $0.9\pm0.4$ \\
\cline{2-11}
& $Z/\gamma^*\rightarrow ee$ & \--- & $9.9\pm0.7$ & $7.5\pm0.6$ & $7.3\pm0.6$ & $1.7\pm0.2$ & $1.4\pm0.2$ & $0.25\pm0.05$ & $0.22\pm0.05$ & $0.06\pm0.02$ \\
& $t\bar{t}$ & \--- & $37\pm7$ & $22\pm4$ & $18\pm3$ & $6\pm2$ & $3.8\pm1.2$ & $0.7\pm0.6$ & $0.7\pm0.6$ & $0.4\pm0.3$ \\
& Single-top (Wt) & \--- & $15.5\pm1.2$ & $9.5\pm0.7$ & $8.0\pm0.6$ & $3.1\pm0.3$ & $2.1\pm0.2$ & $0.45\pm0.09$ & $0.45\pm0.10$ & $0.3\pm0.2$ \\
& Fake electron & \--- & $7.1\pm1.4$ & $3.8\pm0.8$ & $3.4\pm0.7$ & $0.9\pm0.2$ & $0.130\pm0.010$ & \--- & \--- & \--- \\
& Diboson & \--- & $9\pm2$ & $6\pm2$ & $4.5\pm1.3$ & $1.9\pm0.5$ & $1.3\pm0.4$ & $0.38\pm0.13$ & $0.33\pm0.12$ & $0.14\pm0.06$ \\
& $Z/\gamma^*\rightarrow \tau\tau$ & \--- & $0.09\pm0.03$ & $0.030\pm0.010$ & $0.030\pm0.010$ & $0.020\pm0.010$ & \--- & \--- & \--- & \--- \\
			\end{tabular}
		}
	\end{center}
\end{sidewaystable}

